Effective Capacity Analysis of HARQ-enabled D2D Communication in Multi-Tier Cellular Networks

This work does the statistical quality-of-service (QoS) analysis of a block-fading device-to-device (D2D) link in a multi-tier cellular network that consists of a macro-BS (BSMC) and a micro-BS (BSmC) which both operate in full-duplex (FD) mode. For the D2D link under consideration, we first formulate the mode selection problem-whereby D2D pair could either communicate directly, or, through the BSmC, or, through the BSMC-as a ternary hypothesis testing problem. Next, to compute the effective capacity (EC) for the given D2D link, we assume that the channel state information (CSI) is not available at the transmit D2D node, and hence, it transmits at a fixed rate r with a fixed power. This allows us to model the D2D link as a Markov system with six-states. We consider both overlay and underlay modes for the D2D link. Moreover, to improve the throughput of the D2D link, we assume that the D2D pair utilizes two special automatic repeat request (ARQ) schemes, i.e., Hybrid-ARQ (HARQ) and truncated HARQ. Furthermore, we consider two distinct queue models at the transmit D2D node, based upon how it responds to the decoding failure at the receive D2D node. Eventually, we provide closed-form expressions for the EC for both HARQ-enabled D2D link and truncated HARQ-enabled D2D link, under both queue models. Noting that the EC looks like a quasi-concave function of r, we further maximize the EC by searching for an optimal rate via the gradient-descent method. Simulation results provide us the following insights: i) EC decreases with an increase in the QoS exponent, ii) EC of the D2D link improves when HARQ is employed, iii) EC increases with an increase in the quality of self-interference cancellation techniques used at BSmC and BSMC in FD mode.

==> On the Impact of Mode Selection on Effective Capacity of HARQ-IR enabled D2D Communication (1) (8)/abstract.tex <==
\begin{abstract}

Consider a device-to-device (D2D) link which utilizes the mode selection to decide between the direct mode and cellular mode. This paper investigates the impact of mode selection on effective capacity (EC)--the maximum sustainable constant arrival rate at a transmitter's queue under statistical quality-of-service constraints--of a D2D link for both overlay and underlay scenarios. Due to lack of channel state information, the transmit device sends data at a fixed rate and fixed power; this fact combined with mode selection makes the D2D channel a Markov service process. Thus, the EC is obtained by calculating the entries of the transition probability matrix corresponding to the Markov D2D channel. Numerical results show that the EC decays exponentially (and the gain of overlay D2D over underlay D2D diminishes) with the increase in estimation error of the pathloss measurements utilized by the mode selection.

\end{abstract}



==> On the Impact of Mode Selection on Effective Capacity of HARQ-IR enabled D2D Communication (1) (8)/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

This work investigated the impact of mode selection on the EC of a D2D link. The derived analytical expression of the EC, as well as simulation results, reveal that the EC decreases exponentially fast as the pathloss measurements become more noisy. Thus, designing efficient estimators (of the features considered by the mode selection) meeting the CRB is of paramount importance. Additionally, for fixed $\sigma_T$ and $\theta$, the expression in Eq. (\ref{eq:EC}) further allows us to compute the optimal (fixed) rate $r^*$ which maximizes the EC.


==> On the Impact of Mode Selection on Effective Capacity of HARQ-IR enabled D2D Communication (1) (8)/keywords.tex <==
\begin{keywords}

Effective capacity, D2D communication, Overlay, Inband, 5G

\end{keywords}} 

==> abstract.tex <==
\begin{abstract}

Consider a device-to-device (D2D) link which utilizes the mode selection to decide between the direct mode and cellular mode. This paper investigates the impact of mode selection on effective capacity (EC)--the maximum sustainable constant arrival rate at a transmitter's queue under statistical quality-of-service constraints--of a D2D link for both overlay and underlay scenarios. Due to lack of channel state information, the transmit device sends data at a fixed rate and fixed power; this fact combined with mode selection makes the D2D channel a Markov service process. Thus, the EC is obtained by calculating the entries of the transition probability matrix corresponding to the Markov D2D channel. Numerical results show that the EC decays exponentially (and the gain of overlay D2D over underlay D2D diminishes) with the increase in estimation error of the pathloss measurements utilized by the mode selection.

\end{abstract}



==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

This work investigated the impact of mode selection on the EC of a D2D link. The derived analytical expression of the EC, as well as simulation results, reveal that the EC decreases exponentially fast as the pathloss measurements become more noisy. Thus, designing efficient estimators (of the features considered by the mode selection) meeting the CRB is of paramount importance. Additionally, for fixed $\sigma_T$ and $\theta$, the expression in Eq. (\ref{eq:EC}) further allows us to compute the optimal (fixed) rate $r^*$ which maximizes the EC.


==> keywords.tex <==
\begin{keywords}

Effective capacity, D2D communication, Overlay, Inband, 5G

\end{keywords}} 
